Review of Inductive Pulsed Power Generators for Railguns

This literature review addresses inductive pulsed power generators and their major components. Different inductive storage designs like solenoids, toroids and force-balanced coils are briefly presented and their advantages and disadvantages are mentioned. Special emphasis is given to inductive circuit topologies which have been investigated in railgun research such as the XRAM, meat grinder or pulse transformer topologies. One section deals with opening switches as they are indispensable for inductive storages and another one deals briefly with SMES for pulsed power applications. In the end, the most relevant inductor systems which were realized in respect to railgun research are summarized in a table, together with its main characteristics.

==> Figs/Inductive/MEATgrindercircuit2.tex <==
%Figure Meat grinder circuit
%by oliver Liebfried

  \begin{circuitikz}[scale=0.8,american]
    \draw
    (0,0) to [american voltage source,l^=$V_0$](0,2) to [opening switch,l_=$S_o$](0,4) to [L,l^=$L_{1}$,-*](2,4) to [switch,l^=$S_c$,*-*](2,0) to [short,i_=$I_{}$] (0,0);
    \draw (2,4) to [L,l^=$L_{2}$,*-*] (4,4) to [switch,l^=$S_c$,*-*](4,0) to [short] (2,0);
    \draw (4,4) to [L,l^=$L_{3}$,*-*] (6,4) to [switch,l^=$S_c$,*-*](6,0) to [short] (4,0);
    \draw (7,4) to [short] (8,4) to [L,l^=$L_{n}$] (8,1.15)
    (8,0.85) to [short] (8,0) to [short] (7,0);
    \draw[dashed] (6,4) -- (7,4)
    (7,0)  -- (6,0);  
    
    \draw[very thick] (8,1.15) to [short] (10,1.15)
    (8,0.85) to [short] (10,0.85);
    \draw[line width=6pt] (8.5,1.15) -- (8.5,0.85);
    \draw[-latex,semithick] (8.5,1) -- (9,1);
    \draw (9,0.5) node {$Railgun$};
    
    %\draw[-latex,semithick] (0.5,2.4) -- (1.5,2.4);
    %\draw (1,2.6) node {$V_{sw}$};
 \end{circuitikz} 


==> mathsymbols.tex <==
%List of Symbols
%by Oliver Liebfried
%last update: 2016/02/17

\newglossaryentry{W}{
	name={\ensuremath{W}},
	description={energy},
	symbol={\ensuremath{W}}
}

\newglossaryentry{E}{
		name={\ensuremath{E}},
		description={electric field strength},
		symbol={\ensuremath{E}}
}

\newglossaryentry{V}{
		name={\ensuremath{V}},
		description={volume},
		symbol={\ensuremath{V}}
}

\newglossaryentry{epsilonr}{
		name={\ensuremath{\varepsilon_r}},
		description={relative permittivity},
		symbol={\ensuremath{\varepsilon_r}}
}

\newglossaryentry{epsilon0}{
		name={\ensuremath{\varepsilon_0}},
		description={permittivity of vacuum},
		symbol={\ensuremath{\varepsilon_0}}
}

\newglossaryentry{U}{
		name={\ensuremath{U}},
		description={voltage},
		symbol={\ensuremath{U}}
}

\newglossaryentry{d}{
		name={\ensuremath{d}},
		description={thickness},
		symbol={\ensuremath{d}}
}

\newglossaryentry{B}{
		name={\ensuremath{B}},
		description={magnetic flux density},
		symbol={\ensuremath{B}}
}

\newglossaryentry{J}{
		name={\ensuremath{J}},
		description={moment of inertia},
		symbol={\ensuremath{J}}
}

\newglossaryentry{rho}{
		name={\ensuremath{\rho}},
		description={volumetric mass density},
		symbol={\ensuremath{\rho}}
}

\newglossaryentry{r}{
		name={\ensuremath{r}},
		description={radius},
		symbol={\ensuremath{r}}
}

\newglossaryentry{pmag}{
		name={\ensuremath{p_{mag}}},
		description={magnetic pressure},
		symbol={\ensuremath{p_{mag}}}
}

\newglossaryentry{sigma}{
		name={\ensuremath{\sigma_t}},
		description={tensile strength},
		symbol={\ensuremath{\sigma_t}}
}

\newglossaryentry{v}{
		name={\ensuremath{v}},
		description={rim speed},
		symbol={\ensuremath{v}}
}

\newglossaryentry{omega}{
		name={\ensuremath{\omega}},
		description={angular velocity},
		symbol={\ensuremath{\omega}}
}

\newglossaryentry{lR}{
		name={\ensuremath{l_R}},
		description={length of the active rotor region},
		symbol={\ensuremath{l_R}}
}

\newglossaryentry{r1}{
		name={\ensuremath{r1}},
		description={shaft radius},
		symbol={\ensuremath{r1}}
}

\newglossaryentry{r2}{
		name={\ensuremath{r2}},
		description={disc radius},
		symbol={\ensuremath{r2}}
}

\newglossaryentry{C}{
		name={\ensuremath{C}},
		description={capacitance},
		symbol={\ensuremath{C}}
}

\newglossaryentry{t}{
		name={\ensuremath{t}},
		description={time},
		symbol={\ensuremath{t}}
}

\newglossaryentry{n}{
		name={\ensuremath{n}},
		description={number of wire turns},
		symbol={\ensuremath{n}}
}

\newglossaryentry{A}{
		name={\ensuremath{A}},
		description={active area},
		symbol={\ensuremath{A}}
}

\newglossaryentry{M}{
		name={\ensuremath{M}},
		description={mass},
		symbol={\ensuremath{M}}
}

\newglossaryentry{Mmol}{
		name={\ensuremath{M_{mol}}},
		description={molar mass},
		symbol={\ensuremath{M_{mol}}}
}

\newglossaryentry{q}{
		name={\ensuremath{q}},
		description={equivalent per mol},
		symbol={\ensuremath{q}}
}

\newglossaryentry{F}{
		name={\ensuremath{F}},
		description={Faraday constant},
		symbol={\ensuremath{F}}
}

\newglossaryentry{Uth}{
		name={\ensuremath{U_{th}}},
		description={theoretical voltage},
		symbol={\ensuremath{U_{th}}}
}

\newglossaryentry{Vmol}{
		name={\ensuremath{V_{mol}}},
		description={molar volume},
		symbol={\ensuremath{V_{mol}}}
}

\newglossaryentry{mur}{
		name={\ensuremath{\mu_r}},
		description={relative permeability},
		symbol={\ensuremath{\mu_r}}
}

\newglossaryentry{mu0}{
		name={\ensuremath{\mu_0}},
		description={permeability of vaccum},
		symbol={\ensuremath{\mu_0}}
}

\newglossaryentry{I}{
		name={\ensuremath{I}},
		description={current},
		symbol={\ensuremath{I}}
}

\newglossaryentry{L}{
		name={\ensuremath{L}},
		description={inductance},
		symbol={\ensuremath{L}}
}

\newglossaryentry{R}{
		name={\ensuremath{R}},
		description={resistance},
		symbol={\ensuremath{R}}
}

\newglossaryentry{N1}{
		name={\ensuremath{N_1}},
		description={number of primary transformer windings},
		symbol={\ensuremath{N_1}}
}

\newglossaryentry{N2}{
		name={\ensuremath{N_2}},
		description={number of secondary transformer windings},
		symbol={\ensuremath{N_2}}
}
